SEIL: Simulation-augmented Equivariant Imitation Learning

In robotic manipulation, acquiring samples is extremely expensive because it often requires interacting with the real world. Traditional image-level data augmentation has shown the potential to improve sample efficiency in various machine learning tasks. However, image-level data augmentation is insufficient for an imitation learning agent to learn good manipulation policies in a reasonable amount of demonstrations. We propose Simulation-augmented Equivariant Imitation Learning (SEIL), a method that combines a novel data augmentation strategy of supplementing expert trajectories with simulated transitions and an equivariant model that exploits the $\mathrm{O}(2)$ symmetry in robotic manipulation. Experimental evaluations demonstrate that our method can learn non-trivial manipulation tasks within ten demonstrations and outperforms the baselines with a significant margin.

==> dian_working.tex <==
We define $\Pi: (C, p, \lambda) \mapsto I\in \mathbb{R}^{h\times w}$ as an observation projection function that projects a point cloud into an orthographic projection depth image centered at $(x, y, z)$ with a gripper at the center of the image with an orientation $\theta$ and open width $\lambda$ (Figure~\ref{}).
